Alleviating Label Switching with Optimal Transport

Label switching is a phenomenon arising in mixture model posterior inference that prevents one from meaningfully assessing posterior statistics using standard Monte Carlo procedures. This issue arises due to invariance of the posterior under actions of a group; for example, permuting the ordering of mixture components has no effect on the likelihood. We propose a resolution to label switching that leverages machinery from optimal transport. Our algorithm efficiently computes posterior statistics in the quotient space of the symmetry group. We give conditions under which there is a meaningful solution to label switching and demonstrate advantages over alternative approaches on simulated and real data.

==> motivation.tex <==
\section{Motivation}
\label{sec:motivation}

\seb{I don't know if this section needs to exist separately, but this info has to appear somewhere in the paper before \S\ref{sec:theory}}

Let's consider the following abstracted version of our problem. We are given a metric space of parameters $(X, d)$ and a group $G$ that acts by isometry on $X$ (i.e. such that $d(x, y) = d(g\cdot x, g\cdot y)$ for all $g\in G$. We run an inference procedure on a mixture model and receive samples $x \in X$, but suffer from an identifiability issue in that samples $x$ and $g\cdot x$ are indistinguishable by the model.

The lack of identifiability induces a probability distribution on $X$ given by the orbit of $x$ under $G$: 
\begin{align*}
    \mu_x = \sum_{g\in G} \delta_{g\cdot x}.
\end{align*}
We wish to obtain meaningful statistics for the samples $x_1, \ldots, x_n$, but a naive Euclidean average can lead to incorrect results.

To recover meaningful estimates, we must operate on orbits of samples in a way that aligns samples to the correct region of the posterior density. To approach this problem, we leverage the theory of optimal transport and the notion of a Wasserstein barycenter. 

\subsection{Optimal Transport}
Given two distributions $\mu$, $\nu$ supported on $X$ with associated cost $c(\cdot, \cdot)$, the optimal transport cost between $\mu$ and $\nu$ is given by an optimization problem
\begin{align*}
    \inf_{\pi \in \Pi(\mu, \nu)} \int_{X\times X} c(x, y)\mathrm{d}\pi(x, y)
\end{align*}
where $\Pi(\mu, \nu)$ is the set of couplings between measures $\mu$ and $\nu$. When the cost is a power of the metric, the optimal transport solution induces a metric on the space $\mathcal{P}(X)$ of measures on $X$ that is more commonly referred to as the Wasserstein distance $W_p$ (CITE).

The Wasserstein distance turns $\mathcal{P}(X)$ into a metric space, and we can define a notion of a barycenter of measures $\nu_1, \ldots, \nu_n$ as the Fr\'echet mean (CITE)
\begin{align*}
    \nu = \argmin_{\nu\in \mathcal{P}(X)} \sum_{i=1}^n \frac{1}{n} W_p^p(\nu, \nu_i).
\end{align*}


==> problem.tex <==
\section{Problem definition}
We focus our attention on sampling-based posterior approximation in Bayesian modeling. Let $\Theta$ denote all parameters in the model and $X=\{x_1,\ldots,x_N\}$ observed data points. Our goal is to approximate the posterior $p(\Theta|X) \approx \frac{1}{M}\sum_{m=1}^M \delta_{\Theta_m}$, where $\Theta_m \sim p(\Theta|X)$ for $m=1,\ldots,M$. In words, as the posterior is often not tractable analytically, we estimate it using an empirical distribution of $M$ (posterior) samples. Such samples may be obtained using MCMC or more modern approaches such as Hamiltonian Monte Carlo (HMC) \citep{betancourt2017conceptual} amongst others. For HMC, probabilistic programming software Stan \citep{carpenter2017stan} offers a convenient modeling interface.

It is typical for many Bayesian models, e.g., mixture models, Hierarchical Markov Models (HMM) and LDA, to prefer weakly informative exchangeable priors. \ed{What is weakly informative? The likelihood also needs to satisfy some symmetry for the posterior to be group-invariant, no?} This unfortunately leads to the identifiability problem known as \emph{label switching}. For illustration, consider mixture model with $\Theta = \{\theta_1,\ldots,\theta_K\}$, where $\theta_k = \{\mu_k,\pi_k\}$ parameters and probability of the corresponding mixture component with exchangeable priors, and data-generating mechanism
\begin{equation}
\label{eq_gaus_mixture}
p(x|\Theta) = \sum_{k=1}^K \pi_k f(x;\mu_k).
\end{equation}
\ed{Should probably throw in a stem about what $f$ denotes (presumably a Gaussian or some other component model distribution)?}
For any permutation $\sigma(\cdot)$ of labels $k=1,\ldots,K$ let $\sigma(\Theta) = \{\theta_{\sigma(1)},\ldots,\theta_{\sigma(K)}\}$ and observe that
\begin{equation*}
  p(x|\sigma(\Theta)) = \sum_{k=1}^K \pi_{\sigma(k)} f(x;\mu_{\sigma(k)}) = p(x|\Theta).
\end{equation*}
Permutation invariance of the data-generating mechanism implies $K!$ symmetric regions in the posterior of $\Theta$ --- one for each possible permutation of the labels. This phenomena makes it challenging to obtain meaningful parameter statistics (e.g. means and variances of the mixture components) from the generated posterior samples as they may belong to different symmetric regions of the posterior invalidating classic Monte Carlo averaging. \ed{Dumb question: what is this? Just standard averaging? Or is it approximation with multiple support points? If so, how are these points obtained?}

Let $m$-th sample $\Theta_m$ be a $K \times J$ matrix with each row corresponding to sampled parameters of the mixture components (e.g. if $\mu_k$ is the mean and $D$ is the data dimension, $J=D+K$). \ed{Shouldn't this be $D+1$, with an additional entry for the weight of the component? why the additional $K$ entries?} Our goal is to find permutations $\sigma_m(\cdot)$ for $m=1,\ldots,M$ such that when applied to rows of the samples they become aligned allowing subsequent Monte Carlo based estimation. There seems to be no common objective function for finding these permutations, however it is possible to cast it as an optimization problem, which we will discuss later.
